Scalable In-Context Learning on Tabular Data via Retrieval-Augmented Large Language Models

Recent studies have shown that large language models (LLMs), when customized with post-training on tabular data, can acquire general tabular in-context learning (TabICL) capabilities. These models are able to transfer effectively across diverse data schemas and different task domains. However, existing LLM-based TabICL approaches are constrained to few-shot scenarios due to the sequence length limitations of LLMs, as tabular instances represented in plain text consume substantial tokens. To address this limitation and enable scalable TabICL for any data size, we propose retrieval-augmented LLMs tailored to tabular data. Our approach incorporates a customized retrieval module, combined with retrieval-guided instruction-tuning for LLMs. This enables LLMs to effectively leverage larger datasets, achieving significantly improved performance across 69 widely recognized datasets and demonstrating promising scaling behavior. Extensive comparisons with state-of-the-art tabular models reveal that, while LLM-based TabICL still lags behind well-tuned numeric models in overall performance, it uncovers powerful algorithms under limited contexts, enhances ensemble diversity, and excels on specific datasets. These unique properties underscore the potential of language as a universal and accessible interface for scalable tabular data learning.

==> tables/datasets-stats-all.tex <==
\begin{table}[]
\caption{Benchmark dataset statistics}
\scalebox{0.95}{
\begin{tabular}{rllrrrr}
\toprule
\multicolumn{1}{l}{ID} & Source       & Dataset name                                     & \multicolumn{1}{l}{Row} & \multicolumn{1}{l}{Cls} & \multicolumn{1}{l}{Num} & \multicolumn{1}{l}{Cat} \\
\toprule
1                      & GTL-KDD    & alcohol-effects-on-study                         & 1044                    & -1                      & 5                       & 17                      \\
2                      & GTL-KDD    & airfoil-selfnoise-dataset                        & 1503                    & -1                      & 5                       & 0                       \\
3                      & GTL-KDD    & abalone-age-prediction                           & 3550                    & -1                      & 7                       & 3                       \\
4                      & GTL-KDD    & dummy-advertising-and-sales-data                 & 4566                    & -1                      & 3                       & 1                       \\
5                      & GTL-KDD    & co2-emission-by-vehicles                         & 7385                    & -1                      & 6                       & 5                       \\
6                      & GTL-KDD    & melody-metrics-decoding-song-popularity          & 8020                    & -1                      & 5                       & 1                       \\
7                      & GTL-KDD    & crop-yield-in-indian-states-dataset              & 19689                   & -1                      & 6                       & 3                       \\
8                      & GTL-KDD    & car-prices-poland                                & 117927                  & -1                      & 3                       & 6                       \\
9                      & GTL-KDD    & go-to-college-dataset                            & 1000                    & 2                       & 4                       & 6                       \\
10                     & GTL-KDD    & telecom-churn-datasets                           & 3333                    & 2                       & 15                      & 4                       \\
11                     & GTL-KDD    & stroke-prediction-dataset                        & 5110                    & 2                       & 3                       & 7                       \\
12                     & GTL-KDD    & predicting-credit-card-customer-attrition-with-m & 10127                   & 2                       & 14                      & 5                       \\
13                     & GTL-KDD    & datasets-in-it-ops-applied-ai                    & 1000                    & 3                       & 3                       & 4                       \\
14                     & GTL-KDD    & maternal-health-risk-data                        & 1014                    & 3                       & 6                       & 0                       \\
15                     & GTL-KDD    & iris-dataset-extended                            & 1200                    & 3                       & 19                      & 1                       \\
16                     & GTL-KDD    & stellar-classification-dataset-sdss17            & 100000                  & 3                       & 9                       & 6                       \\
17                     & GTL-KDD    & factors-affecting-children-anemia-level          & 13136                   & 4                       & 4                       & 11                      \\
\midrule
18                     & TabR-ICLR    & adult                                            & 26048                   & 2                       & 6                       & 8                       \\
19                     & TabR-ICLR    & higgs-small                                      & 62751                   & 2                       & 28                      & 0                       \\
20                     & TabR-ICLR    & otto                                             & 39601                   & 9                       & 93                      & 0                       \\
21                     & TabR-ICLR    & covtype                                          & 62751                   & 7                       & 10                      & 44                      \\
22                     & TabR-ICLR    & black-friday                                     & 100000                  & -1                      & 4                       & 5                       \\
23                     & TabR-ICLR    & house                                            & 14581                   & -1                      & 16                      & 0                       \\
24                     & TabR-ICLR    & microsoft                                        & 100000                  & -1                      & 131                     & 5                       \\
25                     & TabR-ICLR    & weather-small                                    & 100000                  & -1                      & 118                     & 1                       \\
\midrule
26                     & Tree-NeurIPS & road-safety                                      & 50000                   & 2                       & 29                      & 3                       \\
27                     & Tree-NeurIPS & upselling                                        & 3589                    & 2                       & 34                      & 15                      \\
28                     & Tree-NeurIPS & compass                                          & 10000                   & 2                       & 8                       & 9                       \\
29                     & Tree-NeurIPS & electricity                                      & 10000                   & 2                       & 7                       & 1                       \\
30                     & Tree-NeurIPS & rl                                               & 3479                    & 2                       & 5                       & 7                       \\
31                     & Tree-NeurIPS & MiniBooNE                                        & 50000                   & 2                       & 50                      & 0                       \\
32                     & Tree-NeurIPS & jannis                                           & 40306                   & 2                       & 54                      & 0                       \\
33                     & Tree-NeurIPS & credit                                           & 10000                   & 2                       & 10                      & 0                       \\
34                     & Tree-NeurIPS & ipums\_la\_97-small                              & 3631                    & 2                       & 20                      & 0                       \\
35                     & Tree-NeurIPS & phoneme                                          & 2220                    & 2                       & 5                       & 0                       \\
36                     & Tree-NeurIPS & SGEMM\_GPU\_kernel\_performance                  & 50000                   & -1                      & 3                       & 6                       \\
37                     & Tree-NeurIPS & nyc-taxi-green-dec-2016                          & 50000                   & -1                      & 9                       & 7                       \\
38                     & Tree-NeurIPS & particulate-matter-ukair-2017                    & 50000                   & -1                      & 3                       & 3                       \\
39                     & Tree-NeurIPS & Brazilian\_houses                                & 7484                    & -1                      & 8                       & 3                       \\
40                     & Tree-NeurIPS & OnlineNewsPopularity                             & 9999                    & -1                      & 45                      & 14                      \\
41                     & Tree-NeurIPS & analcatdata\_supreme                             & 2836                    & -1                      & 2                       & 5                       \\
42                     & Tree-NeurIPS & house\_sales                                     & 10000                   & -1                      & 15                      & 2                       \\
43                     & Tree-NeurIPS & visualizing\_soil                                & 6048                    & -1                      & 3                       & 1                       \\
44                     & Tree-NeurIPS & yprop\_4\_1                                      & 6219                    & -1                      & 42                      & 20                      \\
45                     & Tree-NeurIPS & year                                             & 50000                   & -1                      & 90                      & 0                       \\
46                     & Tree-NeurIPS & Ailerons                                         & 9625                    & -1                      & 33                      & 0                       \\
47                     & Tree-NeurIPS & MiamiHousing2016                                 & 9752                    & -1                      & 13                      & 0                       \\
48                     & Tree-NeurIPS & cpu\_act                                         & 5734                    & -1                      & 21                      & 0                       \\
49                     & Tree-NeurIPS & elevators                                        & 10000                   & -1                      & 16                      & 0                       \\
50                     & Tree-NeurIPS & fifa                                             & 10000                   & -1                      & 5                       & 0                       \\
51                     & Tree-NeurIPS & houses                                           & 10000                   & -1                      & 8                       & 0                       \\
52                     & Tree-NeurIPS & medical\_charges                                 & 10000                   & -1                      & 3                       & 0                       \\
53                     & Tree-NeurIPS & pol                                              & 10000                   & -1                      & 26                      & 0                       \\
54                     & Tree-NeurIPS & sulfur                                           & 7056                    & -1                      & 6                       & 0                       \\
55                     & Tree-NeurIPS & superconduct                                     & 10000                   & -1                      & 79                      & 0                   \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/datastats-default8.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lrrrr@{}}
\toprule
Name                           & \multicolumn{1}{l}{Row} & \multicolumn{1}{l}{Cls} & \multicolumn{1}{l}{Num Feat} & \multicolumn{1}{l}{Cat Feat} \\ \midrule
House 16H (house)              & 19138                   & -1                      & 16                           & 0                            \\
Black Friday (black-friday)    & 101000                  & -1                      & 4                            & 5                            \\
Shifts Weather (weather-small) & 101000                  & -1                      & 118                          & 1                            \\
Microsoft (microsoft)          & 101000                  & -1                      & 131                          & 5                            \\
Adult (adult)                  & 27048                   & 2                       & 6                            & 9                            \\
Higgs Small (higgs-small)      & 63751                   & 2                       & 28                           & 0                            \\
Otto Group Products (otto)     & 40601                   & 9                       & 93                           & 0                            \\
Covertype (covtype)            & 101000                  & 7                       & 54                           & 44                           \\ \bottomrule
\end{tabular}
\end{table}

==> tables/datastats-kdd18.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lrrrr@{}}
\toprule
Name                                                   & \multicolumn{1}{l}{Row} & \multicolumn{1}{l}{Cls} & \multicolumn{1}{l}{Num Feat} & \multicolumn{1}{l}{Cat Feat} \\ \midrule
alcohol-effects-on-study (url)                         & 1044                    & -1                      & 5                            & 17                           \\
airfoil-selfnoise-dataset (url)                        & 1503                    & -1                      & 5                            & 0                            \\
abalone-age-prediction (url)                           & 3550                    & -1                      & 7                            & 3                            \\
dummy-advertising-and-sales-data (url)                 & 4566                    & -1                      & 3                            & 1                            \\
co2-emission-by-vehicles (url)                         & 7385                    & -1                      & 6                            & 5                            \\
melody-metrics-decoding-song-popularity (url)          & 8020                    & -1                      & 5                            & 1                            \\
crop-yield-in-indian-states-dataset (url)              & 19689                   & -1                      & 6                            & 3                            \\
car-prices-poland (url)                                & 117927                  & -1                      & 3                            & 6                            \\
go-to-college-dataset (url)                            & 1000                    & 2                       & 4                            & 6                            \\
telecom-churn-datasets (url)                           & 3333                    & 2                       & 15                           & 4                            \\
stroke-prediction-dataset (url)                        & 5110                    & 2                       & 3                            & 7                            \\
predicting-credit-card-customer-attrition-with-m (url) & 10127                   & 2                       & 14                           & 5                            \\
bank-account-fraud-dataset-neurips-2022 (url)          & 1000000                 & 2                       & 19                           & 12                           \\
datasets-in-it-ops-applied-ai (url)                    & 1000                    & 3                       & 3                            & 4                            \\
maternal-health-risk-data (url)                        & 1014                    & 3                       & 6                            & 0                            \\
iris-dataset-extended (url)                            & 1200                    & 3                       & 19                           & 1                            \\
stellar-classification-dataset-sdss17 (url)            & 100000                  & 3                       & 9                            & 6                            \\
factors-affecting-children-anemia-level (url)          & 13136                   & 4                       & 4                            & 11                           \\ \bottomrule
\end{tabular}
\end{table}

==> tables/datastats-tree36.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lrrrr@{}}
\toprule
Name                                                           & \multicolumn{1}{l}{Row} & \multicolumn{1}{l}{Cls} & \multicolumn{1}{l}{Num Feat} & \multicolumn{1}{l}{Cat Feat} \\ \midrule
classif-cat-large-0-covertype                                  & 101000                  & 2                       & 10                           & 44                           \\
classif-cat-large-0-road-safety                                & 101000                  & 2                       & 29                           & 3                            \\
classif-cat-medium-0-KDDCup09\_upselling                       & 5124                    & 2                       & 34                           & 15                           \\
classif-cat-medium-0-compass                                   & 16643                   & 2                       & 8                            & 9                            \\
classif-cat-medium-0-electricity                               & 38474                   & 2                       & 7                            & 1                            \\
classif-cat-medium-0-rl                                        & 4967                    & 2                       & 5                            & 7                            \\
classif-num-large-0-Higgs                                      & 101000                  & 2                       & 24                           & 0                            \\
classif-num-large-0-MiniBooNE                                  & 72998                   & 2                       & 50                           & 0                            \\
classif-num-large-0-jannis                                     & 57580                   & 2                       & 54                           & 0                            \\
classif-num-medium-0-credit                                    & 16714                   & 2                       & 10                           & 0                            \\
classif-num-medium-0-kdd\_ipums\_la\_97-small                  & 5188                    & 2                       & 20                           & 0                            \\
classif-num-medium-0-phoneme                                   & 3172                    & 2                       & 5                            & 0                            \\
regression-cat-large-0-SGEMM\_GPU\_kernel\_performance         & 101000                  & -1                      & 3                            & 6                            \\
regression-cat-large-0-black\_friday                           & 101000                  & -1                      & 4                            & 5                            \\
regression-cat-large-0-nyc-taxi-green-dec-2016                 & 101000                  & -1                      & 9                            & 7                            \\
regression-cat-large-0-particulate-matter-ukair-2017           & 101000                  & -1                      & 3                            & 3                            \\
regression-cat-medium-0-Brazilian\_houses                      & 10692                   & -1                      & 8                            & 3                            \\
regression-cat-medium-0-Mercedes\_Benz\_Greener\_Manufacturing & 4209                    & -1                      & 0                            & 359                          \\
regression-cat-medium-0-OnlineNewsPopularity                   & 39644                   & -1                      & 45                           & 14                           \\
regression-cat-medium-0-analcatdata\_supreme                   & 4052                    & -1                      & 2                            & 5                            \\
regression-cat-medium-0-house\_sales                           & 21613                   & -1                      & 15                           & 2                            \\
regression-cat-medium-0-visualizing\_soil                      & 8641                    & -1                      & 3                            & 1                            \\
regression-cat-medium-0-yprop\_4\_1                            & 8885                    & -1                      & 42                           & 20                           \\
regression-num-large-0-year                                    & 101000                  & -1                      & 90                           & 0                            \\
regression-num-medium-0-Ailerons                               & 13750                   & -1                      & 33                           & 0                            \\
regression-num-medium-0-MiamiHousing2016                       & 13932                   & -1                      & 13                           & 0                            \\
regression-num-medium-0-cpu\_act                               & 8192                    & -1                      & 21                           & 0                            \\
regression-num-medium-0-elevators                              & 16599                   & -1                      & 16                           & 0                            \\
regression-num-medium-0-fifa                                   & 18063                   & -1                      & 5                            & 0                            \\
regression-num-medium-0-house\_16H                             & 22784                   & -1                      & 16                           & 0                            \\
regression-num-medium-0-houses                                 & 20640                   & -1                      & 8                            & 0                            \\
regression-num-medium-0-isolet                                 & 7797                    & -1                      & 613                          & 0                            \\
regression-num-medium-0-medical\_charges                       & 101000                  & -1                      & 3                            & 0                            \\
regression-num-medium-0-pol                                    & 15000                   & -1                      & 26                           & 0                            \\
regression-num-medium-0-sulfur                                 & 10081                   & -1                      & 6                            & 0                            \\
regression-num-medium-0-superconduct                           & 21263                   & -1                      & 79                           & 0                            \\ \bottomrule
\end{tabular}
\end{table}

==> tables/perf-overall-kdd.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\caption{Detailed results for GTL benchmark datasets}
\scalebox{0.9}{
\begin{tabular}{@{}llrrrrrrr@{}}
\toprule
ID                     & Metrics & \multicolumn{1}{l}{LR} & \multicolumn{1}{l}{KNN} & \multicolumn{1}{l}{Catboost} & \multicolumn{1}{l}{XGBoost} & TabPFN\_CTX & TabPFN\_Full & \multicolumn{1}{l}{TabRAG} \\ \midrule
\multicolumn{1}{r}{1}  & NRMSE   & 0.1445                 & 0.3797                  & 0.1357                       & 0.1494                      & -           & -            & 0.1477                     \\
                       & NMAE    & 0.0877                 & 0.2766                  & 0.0857                       & 0.0904                      & -           & -            & 0.0742                     \\
\multicolumn{1}{r}{2}  & NRMSE   & 0.0376                 & 0.0616                  & 0.0134                       & 0.0125                      & -           & -            & 0.0287                     \\
                       & NMAE    & 0.0290                 & 0.0524                  & 0.0087                       & 0.0078                      & -           & -            & 0.0218                     \\
\multicolumn{1}{r}{3}  & NRMSE   & 0.2429                 & 0.4152                  & 0.2322                       & 0.2492                      & -           & -            & 0.3057                     \\
                       & NMAE    & 0.1745                 & 0.2969                  & 0.1627                       & 0.1741                      & -           & -            & 0.1995                     \\
\multicolumn{1}{r}{4}  & NRMSE   & 0.0203                 & 0.5124                  & 0.0190                       & 0.0273                      & -           & -            & 0.0687                     \\
                       & NMAE    & 0.0144                 & 0.4389                  & 0.0142                       & 0.0158                      & -           & -            & 0.0508                     \\
\multicolumn{1}{r}{5}  & NRMSE   & 0.0671                 & 0.2391                  & 0.0097                       & 0.0092                      & -           & -            & 0.0291                     \\
                       & NMAE    & 0.0439                 & 0.1818                  & 0.0074                       & 0.0065                      & -           & -            & 0.0080                     \\
\multicolumn{1}{r}{6}  & NRMSE   & 0.0927                 & 0.3963                  & 0.0970                       & 0.1040                      & -           & -            & 0.2460                     \\
                       & NMAE    & 0.0749                 & 0.3220                  & 0.0786                       & 0.0844                      & -           & -            & 0.1963                     \\
\multicolumn{1}{r}{7}  & NRMSE   & 13.5967                & 14.1821                 & 0.4958                       & 0.1786                      & -           & -            & 0.2437                     \\
                       & NMAE    & 3.3334                 & 0.9862                  & 0.1256                       & 0.0330                      & -           & -            & 0.0253                     \\
\multicolumn{1}{r}{8}  & NRMSE   & 0.8164                 & 1.3813                  & 0.2601                       & 0.2500                      & -           & -            & 0.3112                     \\
                       & NMAE    & 0.4732                 & 0.7431                  & 0.1341                       & 0.1328                      & -           & -            & 0.1321                     \\
\midrule
\multicolumn{1}{r}{9}  & ACC     & 0.7070                 & 0.5391                  & 0.9141                       & 0.8828                      & 0.7344      & 0.9102       & 0.9023                     \\
                       & ROCAUC  & 0.8198                 & 0.5000                  & 0.9811                       & 0.9706                      & 0.8588      & 0.9692       & 0.9684                     \\
\multicolumn{1}{r}{10} & ACC     & 0.8203                 & 0.8320                  & 0.9375                       & 0.9297                      & 0.8359      & 0.9258       & 0.8320                     \\
                       & ROCAUC  & 0.7137                 & 0.5000                  & 0.8184                       & 0.8239                      & 0.5900      & 0.8481       & 0.7918                     \\
\multicolumn{1}{r}{11} & ACC     & 0.9492                 & 0.9453                  & 0.9414                       & 0.9375                      & 0.9453      & 0.9453       & 0.9453                     \\
                       & ROCAUC  & 0.8244                 & 0.5000                  & 0.8737                       & 0.8498                      & 0.5682      & 0.8604       & 0.7935                     \\
\multicolumn{1}{r}{12} & ACC     & 0.9844                 & 0.8320                  & 1.0000                       & 1.0000                      & 0.8398      & 1.0000       & 0.9922                     \\
                       & ROCAUC  & 0.9934                 & 0.5000                  & 1.0000                       & 1.0000                      & 0.7976      & 1.0000       & 1.0000                     \\
\multicolumn{1}{r}{13} & ACC     & 0.8281                 & 0.3555                  & 0.8555                       & 0.8555                      & 0.5469      & 0.8633       & 0.7969                     \\
                       & ROCAUC  & 0.9380                 & 0.5000                  & 0.9670                       & 0.9683                      & 0.8308      & 0.9632       & 0.9369                     \\
\multicolumn{1}{r}{14} & ACC     & 0.5781                 & 0.2188                  & 0.8438                       & 0.8516                      & 0.2773      & 0.7813       & 0.8203                     \\
                       & ROCAUC  & 0.7306                 & 0.5000                  & 0.9498                       & 0.9565                      & 0.6883      & 0.9125       & 0.9272                     \\
\multicolumn{1}{r}{15} & ACC     & 0.9922                 & 0.3125                  & 0.9883                       & 0.9844                      & 0.9727      & 0.9922       & 0.9492                     \\
                       & ROCAUC  & 1.0000                 & 0.5000                  & 0.9998                       & 0.9998                      & 0.9995      & 1.0000       & 0.9932                     \\
\multicolumn{1}{r}{16} & ACC     & 0.5898                 & 0.5898                  & 0.9844                       & 0.9805                      & 0.9800      & OOM          & 0.9648                     \\
                       & ROCAUC  & 0.5607                 & 0.5000                  & 0.9922                       & 0.9939                      & 0.9910      & OOM          & 0.9877                     \\ \bottomrule
\end{tabular}
}
\end{table}
